Citadel: Protecting Data Privacy and Model Confidentiality for Collaborative Learning with SGX

With the advancement of machine learning (ML) and its growing awareness, many organizations who own data but not ML expertise (data owner) would like to pool their data and collaborate with those who have expertise but need data from diverse sources to train truly generalizable models (model owner). In such collaborative ML, the data owner wants to protect the privacy of its training data, while the model owner desires the confidentiality of the model and the training method which may contain intellectual properties. However, existing private ML solutions, such as federated learning and split learning, cannot meet the privacy requirements of both data and model owners at the same time. This paper presents Citadel, a scalable collaborative ML system that protects the privacy of both data owner and model owner in untrusted infrastructures with the help of Intel SGX. Citadel performs distributed training across multiple training enclaves running on behalf of data owners and an aggregator enclave on behalf of the model owner. Citadel further establishes a strong information barrier between these enclaves by means of zero-sum masking and hierarchical aggregation to prevent data/model leakage during collaborative training. Compared with the existing SGX-protected training systems, Citadel enables better scalability and stronger privacy guarantees for collaborative ML. Cloud deployment with various ML models shows that Citadel scales to a large number of enclaves with less than 1.73X slowdown caused by SGX.

==> 03charac.tex <==
%!TEX root = main.tex
\section{Characterizing the Single Enclave Design}
\label{sec:charc}

In this section, we present a single enclave prototype that guarantees both model and privacy at the same time, and characterize its performance overhead.

\subsection{The Single Enclave Design}

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{single-enclave.eps}
    \caption{An illustration of a single enclave approach to protect both data and model privacy}
    \label{fig:enclave}
    \vspace{-.1in}
\end{figure}

Earlier works have explored utilizing a single enclave to protect private data during collaborative ML training~\cite{hynes2018efficient}.
Under such scenario, the data owners also devise and own the model together, but with some augmentations, such design can support model privacy for third-party model owner as well.
We present the straw man solution in Fig.~\ref{fig:enclave}.

As seen in Fig.~\ref{fig:enclave}, model and data owners hold their respective secrets (model or data) locally, and the training will take place in an enclave running on an untrusted host machine.
Before training starts, model and data owners generate their own encryption keys, and encrypt their model or data individually.
These encrypted data and model are then uploaded to a storage service running on the unprotected scope of the host machine.
Since the host machine does not process the keys, the secrets are safe.
Then, an enclave is established using an image provided by model and data owners.
The image contains ML codes that are agreed by all model and data owners, so that they are sure that the codes do not leak any of their secrets.
After the enclave is set up, each of the secret owners attests the enclave, ensuring enclave's integrity and correctness.
Once a secret owner establishes trust over the enclave, it uploads its encryption key to the enclave over TLS protected channel.
Following gathering all encryption keys, the enclave can retrieve the encrypted secrets from the storage service, and decrypt them.
Now that the data, model, and ML codes all reside in the enclave, the training is started.
As soon as the training finishes, the trained model is sent to the model owner over the TLS secured channel.
As for model deployment after the training, model owner can choose to deploy it on its own infrastructure privately or on untrusted devices further utilizing TEE~\cite{bayerl2020offline}.


\subsection{Characterization Results}

\begin{figure}
  \centering
  \label{fig:tf_single}
  \subfloat[Training epoch time and slowdown w.r.t. batch size]{
    \includegraphics[width=0.53\columnwidth]{tf_single_slowdown.eps}
    \label{fig:tf_single_slowdown}
  }\hfil
  \subfloat[Memory usage w.r.t. batch size]{
    \includegraphics[width=0.4\columnwidth]{tf_single_mem.eps}
    \label{fig:tf_single_mem}
  }
  \caption{The time needed to finish one epoch training running under SGX and native mode respectively. The slowdown shown in line represents the ratio between SGX time and native time. The memory figure depicts the amount of memory is used actively in SGX.}
  \vspace{-.1in}
\end{figure}

Now that we have outlined the single enclave design, we demonstrate its great performance limitation with performance profiling.
Our characterization is carried out in a realistic setting.
We adopts the largest instance \texttt{Standard\_DC8\_v2} from Azure's latest confidential computing offering \texttt{DCsv2} series~\cite{azure_instance}, a such instance offers 8 vCPUs, 32 GB memory, as well as 168MB of EPC memory.
We train a AlexNet~\cite{krizhevsky2017imagenet} model with TensorSCONE~\cite{kunkel2019tensorscone}, an SGX optimized version of TensorFlow 1.15~\cite{abadi2016tensorflow}.
We have to use TensorSCONE with SGX as the unmodified version of TensorFlow suffers great performance penalty from oblivious memory usage and system calls.
The model is trained with images of size 32*32*3.
We run the same profiling workloads with both TensorSCONE under SGX mode and unmodified TensorFlow on the same instance, respectively, and compare the results.

We summarize and depict our profiling results in Fig~\ref{fig:tf_single_slowdown}.
When batch size is set to 8, we observe a $2.9\times$ slowdown, which matches the optimal performance slowdown claimed by TensorSCONE.
Such slowdown is mainly contributed by SGX's inevitable MEE encryption overhead, as the memory usage now is barely over EPC's size: EPC paging overhead is minimal.
However, as shown in Fig.~\ref{fig:tf_single_mem}, the memory usage keeps hiking up as batch size increases.
Consequentially, the time required to finish an epoch reduces under native mode, as larger batch sizes enable greater parallelism.
Yet, such trend does not stand under SGX mode, the time required to finish an epoch first reduces and then swiftly jumps again with the increase in batch size.
The phenomenon is contributed to the super-linear climb of EPC paging overhead.
As illustrated by the line in Fig.~\ref{fig:tf_single_slowdown}, the slowdown soars to $17.04\times$ when the memory usage climbs thanks to larger batch size.
Even though we still enjoy the benefit from improved parallelism, such speedup becomes trivial compared with the overpowering EPC paging overhead.

Our characterizations show that, even though it is possible to facilitate ML with simply one SGX enclave to protect model and data privacy, we face the tremendous overhead causing a slowdown up to two orders of magnitude.
Because of sophisticated model design and voluminous data, it is typical for a state-of-the-art model to converge in up a a week under native mode alone.
Adding SGX overhead atop time of this kind, it becomes impractical to train complex models with a single SGX enclave.

Besides the significant overhead, the single enclave solution has another issue: to obtain data owner's complete trust, codes running inside the enclave have to be shared.
Even though enclaves prevent data being accessed from outside of the enclaves, a dishonest model owner can still steal information with the codes running inside the enclave.
However, if all the codes were to be shared, parts of model owner's intellectual property has to be compromised (e.g., model update logic).



==> 03threat_old.tex <==
%!TEX root = main.tex
\section{Threat Model}
\label{sec:threat_model}

% \iea{This section needs to come earlier, probably right after intro. It should explicitly state our assumptions. Some subsectional organization would be good here.}

Our goal is to protect data privacy and model confidentiality at the same time
for collaborative ML. For a data owner, it is required that no training data
or model updates are revealed to external entities (i.e., the model owner, cloud provider, and other data owners) in the clear---the same
requirement as in Secure Aggregation~\cite{bonawitz2017practical} and
MPC~\cite{mohassel2017secureml}. For the model owner, we aspire to protect the
intellectual property contained in its model as much as possible.
In addition to ensuring the confidentiality of the model weights, we also want
to conceal the model design and the ML training techniques adopted by the
model owner. These techniques, such as optimizer selection and configuration~\cite{ruder2016overview}, gradient manipulation~\cite{ho2013more,zhang2019gradient} and learning
rate schedule~\cite{zeiler2012adadelta}, are critical to the training performance.
Selecting, combining, and configuring them require extensive ML expertise,
thus should be protected for model owner. 

We assume that data owners and model owner are \emph{honest but curious}. The
data owners might act on their own or collude with each other to steal the training model and the training method so
that they can perform training by their own; they also want to pry on each
other's data for they can be competitors in the same business sector. The
model owner, on the other hand, wants to access the training data for illicit
use. Participants have no incentive to hinder the training and will follow the
training protocols honestly. 

The end system can be deployed on an infrastructure trusted by neither the
data owners nor the model owner. The computing platform, including privileged
softwares like OS and hypervisor, is not trusted. Attacks can be performed by
the infrastructure administrator (e.g., cloud provider) or anyone with access
to the OS or hypervisor. We do not address side-channel
attacks~\cite{van2018foreshadow} and denial-of-service attacks as they can be
prevented~\cite{oleksenko2018varys,baumann2015shielding} and are  out of the
scope of the paper. We also leave out rollback attacks~\cite{parno2011memoir}
on the data stored beyond enclaves, as they can be handled by existing
approaches~\cite{krahn2018pesos,kim2019shieldstore}. Finally, we do not
consider the model owner colluding with some data owners to steal others'
data, as victim data owners can effectively guard against this attack with
differential privacy~\cite{hynes2018efficient}.
% \yanc{how about colluding among data owners to steal the model and/or other data owners' data?}

\paragraph{Trusted Computing Base (TCB)}
For an easy support of SGX and multiple enclave orchestration, we adopt
SCONE~\cite{arnautov2016scone} in our system. SCONE provides SGX-protected
Linux containers, so that we can utilize tools like Docker~\cite{docker} and
Kubernetes~\cite{kubernetes} to orchestrate enclaves. Data owners and model
owner must trust SCONE's codebase, which is provided by a third-part
organization with no conflict of interest. Data and model owners also have to
trust the implementation of Intel SGX and its attestation service. We also assume that the participants trust standard ML
frameworks like TensorFlow~\cite{abadi2016tensorflow} and
PyTorch~\cite{paszke2019pytorch}. These frameworks are developed by reputable
organizations and are under the public scrutiny in open-source communities.


==> 08conclusion.tex <==
%!TEX root = main.tex
%\vspace{-2mm}
\section{Conclusion}
\label{sec:conclusion}

We presented \citadel, the first scalable system for
collaborative machine learning that protects both data privacy and model
confidentiality with SGX. \citadel partitions the training workload into two
parts, the open-sourced data handling code running in training enclaves and
the private model update code running in the aggregator enclave. \citadel
imposes a barrier between the two parts by means of zero-sum masking to prevent data and model leakage and uses a secure hierarchical aggregation scheme to scale up aggregation performance. Experimental results show that \citadel scales to a large number of enclaves at the expense
of a small performance overhead due to SGX.\iea{can we report some numbers here?}

% analyzed the privacy requirements for both model and data owners in collaborative ML.
% We showed that there is no scalable solution to protect data privacy and model confidentiality at the same time.
% To address the problem, we presented \citadel, a scalable system that utilizes SGX to protect interests for all participants.
% We proposed zero-sum masking and hierarchical aggregation to separate codes handling data and model, so that only necessary codes are shared with data owners to gain their trust, while preserving model owner's intellectual property as much as possible.
% We have implemented \citadel and confirmed that \citadel can efficiently speed up training.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes

